Compensation Learning in Semantic Segmentation

Label noise and ambiguities between similar classes are challenging problems in developing new models and annotating new data for semantic segmentation. In this paper, we propose Compensation Learning in Semantic Segmentation, a framework to identify and compensate ambiguities as well as label noise. More specifically, we add a ground truth depending and globally learned bias to the classification logits and introduce a novel uncertainty branch for neural networks to induce the compensation bias only to relevant regions. Our method is employed into state-of-the-art segmentation frameworks and several experiments demonstrate that our proposed compensation learns inter-class relations that allow global identification of challenging ambiguities as well as the exact localization of subsequent label noise. Additionally, it enlarges robustness against label noise during training and allows target-oriented manipulation during inference. We evaluate the proposed method on %the widely used datasets Cityscapes, KITTI-STEP, ADE20k, and COCO-stuff10k.

==> tables/table_qualitative_results_cityscapes_logcomp.tex <==
\begin{table}[t]
    \centering
    \newcommand{\pst}[1]{{\cellcolor{red!\fpeval{100*(#1+0.2)/1.8}}}\scalebox{0.8}{#1}}
    \newcommand{\ngt}[1]{{\cellcolor{blue!\fpeval{100*(#1+0.2)/1.8}}}\scalebox{0.8}{-#1}}
    \newcommand{\zero}[0]{\scalebox{0.6}{0}}
    \newcolumntype{"}{@{\hskip\tabcolsep\vrule width 1pt \hspace{0.1pt}|}}
    \newcolumntype{x}[0]{>{\centering\arraybackslash\hspace{0pt}}p{0.035\textwidth}}
    \caption{Analysis of the correlation weights on Cityscapes. The experiment shows the learned compensation values~$B_{ij}$ for the 11 \textit{stuff} and~8 \textit{thing} classes in~$C$ provided by \textit{LogComp}. A negative value~$B_{ij}$ lowers the impact of class~$i$, if class~$j$ is the ground truth annotation. Positive values increase the impact, respectively. Note that we report the value~$B_{ij}$ rounded after the first digit for readability.}
    \begin{tabular}{c|c|x|x|x|x|x|x|x|x|x|x|x||x|x|x|x|x|x|x|x}
    \toprule
    
\multicolumn{2}{c|}{\multirow{5}{*}{$B_{ij}$}} & \multicolumn{11}{c||}{\textit{stuff}} & \multicolumn{8}{c}{\textit{thing}} \\ \cline{3-21}
    
\multicolumn{2}{c|}{}
& \rotatebox{90}{\textit{road}} 
& \rotatebox{90}{\textit{sidewalk}} 
& \rotatebox{90}{\textit{building}} 
& \rotatebox{90}{\textit{wall}} 
& \rotatebox{90}{\textit{fence}} 
& \rotatebox{90}{\textit{pole}} 
& \rotatebox{90}{\textit{tr. light}}
& \rotatebox{90}{\textit{tr. sign}}
& \rotatebox{90}{\textit{vegetation\ }} 
& \rotatebox{90}{\textit{terrain}} 
& \rotatebox{90}{\textit{sky}} 
& \rotatebox{90}{\textit{person}} 
& \rotatebox{90}{\textit{rider}} 
& \rotatebox{90}{\textit{car}} 
& \rotatebox{90}{\textit{truck}}
& \rotatebox{90}{\textit{bus}}
& \rotatebox{90}{\textit{train}}
& \rotatebox{90}{\textit{motorcycle\ }}
& \rotatebox{90}{\textit{bicycle }} \\\midrule % \hline\hline

\multirow{11}{*}{\rotatebox{90}{\textit{stuff}}}
&\textit{road}      
&\pst{0.5} &\ngt{1.1} &\zero &\ngt{0.2} &\zero &\zero &\zero &\zero &\zero &\ngt{0.5} &\zero 
&\ngt{0.1} &\zero&\zero &\zero &\zero &\zero &\ngt{0.1} &\ngt{0.2} \\\cline{2-2}

&\textit{sidewalk}   
&\zero &\pst{1.3} &\zero &\ngt{0.4} &\ngt{0.3} &\zero &\zero &\zero &\zero &\zero &\zero 
&\zero &\zero&\zero &\zero &\zero &\zero &\zero &\ngt{0.4} \\\cline{2-2}
                    
&\textit{building}   
&\zero &\zero &\pst{1.5} &\ngt{0.7} &\ngt{0.8} &\ngt{1.5} &\ngt{1} &\ngt{1.1} &\ngt{0.7} &\zero &\ngt{0.5} 
&\ngt{1} &\ngt{0.6}&\zero &\ngt{0.4} &\ngt{0.3} &\ngt{0.3} &\ngt{0.4} &\ngt{0.7} \\\cline{2-2}

&\textit{wall}          
&\zero &\zero &\zero &\pst{0.8} &\ngt{0.8} &\zero &\zero &\zero &\zero &\zero &\zero 
&\zero &\zero&\zero &\zero &\zero &\zero &\zero &\zero \\\cline{2-2}
    
&\textit{fence}         
&\zero &\zero &\zero &\ngt{0.8} &\pst{1} &\ngt{0.4} &\zero &\zero &\zero &\zero &\zero 
&\zero &\zero&\zero &\zero &\zero &\ngt{0.1} &\zero &\ngt{0.4} \\\cline{2-2}
    
&\textit{pole}          
&\zero &\zero &\zero &\ngt{0.2} &\ngt{0.5} &\pst{1.6} &\ngt{1} &\ngt{0.6} &\zero &\zero &\zero 
&\zero &\zero&\zero &\zero &\zero &\zero &\zero &\ngt{0.3} \\\cline{2-2}
    
&\textit{tr. light}     
&\zero &\zero &\zero &\zero &\zero &\zero &\pst{1.1} &\zero &\zero &\zero &\zero 
&\zero &\zero&\zero &\zero &\zero &\zero &\zero &\zero \\\cline{2-2}
    
&\textit{tr. sign}     
&\zero &\zero &\zero &\zero &\zero &\zero &\ngt{0.5} &\pst{1.1} &\zero &\zero &\zero 
&\zero &\zero&\zero &\ngt{0.1} &\zero &\zero &\zero &\zero \\\cline{2-2}
    
&\textit{vegetation} 
&\zero &\zero &\ngt{0.3} &\ngt{0.5} &\ngt{0.7} &\ngt{1.3} &\ngt{1} &\ngt{0.9} &1.3 &\zero &\ngt{0.1} 
&\ngt{0.2} &\ngt{0.3}&\zero &\ngt{0.2} &\ngt{0.2} &\zero &\ngt{0.2} &\ngt{0.4} \\\cline{2-2}
    
&\textit{terrain}      
&\zero &\ngt{0.1} &\zero &\ngt{0.3} &\ngt{0.2} &\zero &\zero &\zero &\zero &\pst{0.9} &\zero 
&\zero &\zero&\zero &\zero &\zero &\zero &\zero &\zero \\\cline{2-2}
    
&\textit{sky}      
&\zero &\zero &\zero &\zero &\zero &\zero &\zero &\zero &\zero &\zero &\pst{0.7} 
&\zero &\zero&\zero &\zero &\zero &\zero &\zero &\zero 
\\ \midrule


\multirow{8}{*}{\rotatebox{90}{\textit{thing}}}
&\textit{person}          
&\zero &\zero &\zero &\zero &\ngt{0.1} &\ngt{0.1} &\zero &\zero &\zero &\zero &\zero 
&\pst{1.3} &\ngt{1}&\zero &\ngt{0.1} &\zero &\zero &\ngt{0.5} &\ngt{0.9} \\\cline{2-2}
    
&\textit{rider}      
&\zero &\zero &\zero &\zero &\zero &\zero &\zero &\zero &\zero &\zero &\zero 
&\ngt{0.9} &\pst{1}&\zero &\zero &\zero &\zero &\ngt{0.5} &\ngt{0.7} \\\cline{2-2}
    
&\textit{car}      
&\zero &\zero &\zero &\ngt{0.1} &\ngt{0.3} &\zero &\zero &\ngt{0.1} &\zero &\zero &\zero 
&\ngt{0.6} &\ngt{0.6}&\pst{1.2} &\ngt{0.5} &\ngt{0.4} &\ngt{0.2} &\ngt{0.5} &\ngt{0.7} \\\cline{2-2}
    
&\textit{truck}          
&\zero &\zero &\zero &\zero &\zero &\zero &\zero &\zero &\zero &\zero &\zero 
&\zero &\zero&\zero &\pst{0.5} &\ngt{0.4} &\ngt{0.2} &\zero &\zero \\\cline{2-2}
    
&\textit{bus}         
&\zero &\zero &\zero &\zero &\zero &\zero &\zero &\zero &\zero &\zero &\zero 
&\zero &\zero&\zero &\ngt{0.4} &\pst{0.5} &\ngt{0.4} &\zero &\zero \\\cline{2-2}
    
&\textit{train}         
&\zero &\zero &\zero &\zero &\zero &\zero &\zero &\zero &\zero &\zero &\zero 
&\zero &\zero&\zero &\ngt{0.2} &\ngt{0.4} &\pst{0.4} &\zero &\zero \\\cline{2-2}
    
&\textit{motorcycle}     
&\zero &\zero &\zero &\zero &\zero &\zero &\zero &\zero &\zero &\zero &\zero 
&\zero &\ngt{0.6}&\zero &\zero &\zero &\zero &\pst{0.6} &\ngt{0.7} \\\cline{2-2}
    
&\textit{bicycle}  
&\zero &\zero &\zero &\zero &\zero &\zero &\zero &\zero &\zero &\zero &\zero 
&\zero &\zero&\ngt{0.5} &\ngt{0.9} &\zero &\zero &\ngt{0.6} &\pst{1.1} 
\\\bottomrule

\end{tabular}
\label{tab:qualitative_results_full_cityscapes_logcomp}
\end{table}

==> tables/table_qualitative_results_step_logcomp.tex <==
\begin{table}[t]
    \centering
    \newcommand{\pst}[1]{{\cellcolor{red!\fpeval{100*(#1+0.2)/1.8}}}\scalebox{0.8}{#1}}
    \newcommand{\ngt}[1]{{\cellcolor{blue!\fpeval{100*(#1+0.2)/1.8}}}\scalebox{0.8}{-#1}}
    \newcommand{\zero}[0]{\scalebox{0.6}{0}}
    \newcolumntype{"}{@{\hskip\tabcolsep\vrule width 1pt \hspace{0.1pt}|}}
    \newcolumntype{x}[0]{>{\centering\arraybackslash\hspace{0pt}}p{0.035\textwidth}}
    \caption{Analysis of the correlation weights on KITTI-STEP. The experiment shows the learned compensation values~$B_{ij}$ for the 11 \textit{stuff} and~8 \textit{thing} classes in~$C$ provided by \textit{LogComp}. A negative value~$B_{ij}$ lowers the impact of class~$i$, if class~$j$ is the ground truth annotation. Positive values increase the impact, respectively. Note that we report the value~$B_{ij}$ rounded after the first digit for readability.}
    \begin{tabular}{c|c|x|x|x|x|x|x|x|x|x|x|x||x|x|x|x|x|x|x|x}
    \toprule
    
\multicolumn{2}{c|}{\multirow{5}{*}{$B_{ij}$}} & \multicolumn{11}{c||}{\textit{stuff}} & \multicolumn{8}{c}{\textit{thing}} \\ \cline{3-21}
    
\multicolumn{2}{c|}{}
& \rotatebox{90}{\textit{road}} 
& \rotatebox{90}{\textit{sidewalk}} 
& \rotatebox{90}{\textit{building}} 
& \rotatebox{90}{\textit{wall}} 
& \rotatebox{90}{\textit{fence}} 
& \rotatebox{90}{\textit{pole}} 
& \rotatebox{90}{\textit{tr. light}}
& \rotatebox{90}{\textit{tr. sign}}
& \rotatebox{90}{\textit{vegetation\ }} 
& \rotatebox{90}{\textit{terrain}} 
& \rotatebox{90}{\textit{sky}} 
& \rotatebox{90}{\textit{person}} 
& \rotatebox{90}{\textit{rider}} 
& \rotatebox{90}{\textit{car}} 
& \rotatebox{90}{\textit{truck}}
& \rotatebox{90}{\textit{bus}}
& \rotatebox{90}{\textit{train}}
& \rotatebox{90}{\textit{motorcycle\ }}
& \rotatebox{90}{\textit{bicycle }} \\\midrule % \hline\hline
    
\multirow{11}{*}{\rotatebox{90}{\textit{stuff}}}
&\textit{road}      
&\zero &\zero &\zero &\zero &\zero &\zero &\zero &\zero &\zero &\zero &\zero 
&\zero &\zero&\zero &\zero &\zero &\zero &\zero &\zero \\\cline{2-2}

&\textit{sidewalk}   
&\zero &\zero &\zero &\zero &\zero &\zero &\zero &\zero &\zero &\zero &\zero 
&\zero &\zero&\zero &\zero &\zero &\zero &\zero &\zero \\\cline{2-2}
                    
&\textit{building}   
&\zero &\zero &\zero &\zero &\zero &\zero &\zero &\zero &\zero &\zero &\zero 
&\zero &\zero&\zero &\zero &\zero &\zero &\zero &\zero \\\cline{2-2}

&\textit{wall}          
&\zero &\zero &\zero &\zero &\zero &\zero &\zero &\zero &\zero &\zero &\zero 
&\zero &\zero&\zero &\zero &\zero &\zero &\zero &\zero \\\cline{2-2}
    
&\textit{fence}         
&\zero &\zero &\zero &\zero &\zero &\zero &\zero &\zero &\zero &\zero &\zero 
&\zero &\zero&\zero &\zero &\zero &\zero &\zero &\zero \\\cline{2-2}
    
&\textit{pole}          
&\zero &\zero &\zero &\zero &\zero &\zero &\zero &\zero &\zero &\zero &\zero 
&\zero &\zero&\zero &\zero &\zero &\zero &\zero &\zero \\\cline{2-2}
    
&\textit{tr. light}     
&\zero &\zero &\zero &\zero &\zero &\zero &\zero &\zero &\zero &\zero &\zero 
&\zero &\zero&\zero &\zero &\zero &\zero &\zero &\zero \\\cline{2-2}
    
&\textit{tr. sign}     
&\zero &\zero &\zero &\zero &\zero &\zero &\zero &\zero &\zero &\zero &\zero 
&\zero &\zero&\zero &\zero &\zero &\zero &\zero &\zero \\\cline{2-2}
    
&\textit{vegetation} 
&\zero &\zero &\zero &\zero &\zero &\zero &\zero &\zero &\zero &\zero &\zero 
&\zero &\zero&\zero &\zero &\zero &\zero &\zero &\zero \\\cline{2-2}
    
&\textit{terrain}      
&\zero &\zero &\zero &\zero &\zero &\zero &\zero &\zero &\zero &\zero &\zero 
&\zero &\zero&\zero &\zero &\zero &\zero &\zero &\zero \\\cline{2-2}
    
&\textit{sky}      
&\zero &\zero &\zero &\zero &\zero &\zero &\zero &\zero &\zero &\zero &\zero 
&\zero &\zero&\zero &\zero &\zero &\zero &\zero &\zero 
\\ \midrule


\multirow{8}{*}{\rotatebox{90}{\textit{thing}}}
&\textit{person}          
&\zero &\zero &\zero &\zero &\zero &\zero &\zero &\zero &\zero &\zero &\zero 
&\zero &\zero&\zero &\zero &\zero &\zero &\zero &\zero \\\cline{2-2}
    
&\textit{rider}      
&\zero &\zero &\zero &\zero &\zero &\zero &\zero &\zero &\zero &\zero &\zero 
&\zero &\zero&\zero &\zero &\zero &\zero &\zero &\zero \\\cline{2-2}
    
&\textit{car}      
&\zero &\zero &\zero &\zero &\zero &\zero &\zero &\zero &\zero &\zero &\zero 
&\zero &\zero&\zero &\zero &\zero &\zero &\zero &\zero \\\cline{2-2}
    
&\textit{truck}          
&\zero &\zero &\zero &\zero &\zero &\zero &\zero &\zero &\zero &\zero &\zero 
&\zero &\zero&\zero &\zero &\zero &\zero &\zero &\zero \\\cline{2-2}
    
&\textit{bus}         
&\zero &\zero &\zero &\zero &\zero &\zero &\zero &\zero &\zero &\zero &\zero 
&\zero &\zero&\zero &\zero &\zero &\zero &\zero &\zero \\\cline{2-2}
    
&\textit{train}         
&\zero &\zero &\zero &\zero &\zero &\zero &\zero &\zero &\zero &\zero &\zero 
&\zero &\zero&\zero &\zero &\zero &\zero &\zero &\zero \\\cline{2-2}
    
&\textit{motorcycle}     
&\zero &\zero &\zero &\zero &\zero &\zero &\zero &\zero &\zero &\zero &\zero 
&\zero &\zero&\zero &\zero &\zero &\zero &\zero &\zero \\\cline{2-2}
    
&\textit{bicycle}  
&\zero &\zero &\zero &\zero &\zero &\zero &\zero &\zero &\zero &\zero &\zero 
&\zero &\zero&\zero &\zero &\zero &\zero &\zero &\zero 
\\\bottomrule

\end{tabular}
\label{tab:qualitative_results_full_kitti_logcomp}
\end{table}
